Nuclear-electronic spin systems, magnetic resonance, and quantum information processing

A promising platform for quantum information processing is that of silicon impurities, where the quantum states are manipulated by magnetic resonance. Such systems, in abstraction, can be considered as a nucleus of arbitrary spin coupled to an electron of spin one-half via an isotropic hyperfine interaction. We therefore refer to them as "nuclear-electronic spin systems". The traditional example, being subject to intensive experimental studies, is that of phosphorus doped silicon (Si:P) which couples a spin one-half electron to a nucleus of the same spin, with a hyperfine strength of 117.5 MHz. More recently, bismuth doped silicon (Si:Bi) has been suggested as an alternative instantiation of nuclear-electronic spin systems, differing from Si:P by its larger nuclear spin and hyperfine strength of 9/2 and 1.4754 GHz respectively. The aim of this thesis has been to develop a model that is capable of predicting the magnetic resonance properties of nuclear-electronic spin systems. The theoretical predictions of this model have been tested against experimental data collected on Si:Bi at 4.044 GHz, and have proven quite successful. Furthermore, the larger nuclear spin and hyperfine strength of Si:Bi, compared with that of Si:P, are predicted to offer advantages for quantum information processing. Most notable amongst these is that magnetic field-dependent two-dimensional decoherence free subspaces, called optimal working points, have been identified to exist in Si:Bi, but not Si:P.

==> abstract.tex <==
A promising platform for quantum information processing is that of silicon impurities, where the quantum states are manipulated by magnetic resonance. Such systems, in abstraction, can be considered as a  nucleus of arbitrary spin coupled to an electron of spin one-half via an isotropic hyperfine interaction. We therefore refer to them as "nuclear-electronic spin systems". The traditional example, being subject to intensive experimental studies, is that of phosphorus doped silicon (Si:P) which couples a spin one-half electron to a nucleus of the same spin, with a hyperfine strength of 117.5 MHz. More recently, bismuth doped silicon (Si:Bi) has been suggested as an alternative instantiation of nuclear-electronic spin systems, differing from Si:P by its larger nuclear spin and hyperfine strength of 9/2 and 1.4754 GHz respectively. The aim of this thesis has been to develop a model that is capable of predicting the magnetic resonance properties of nuclear-electronic spin systems. The theoretical predictions of this model have been tested against experimental data collected on Si:Bi at 4.044 GHz, and have proven quite successful. Furthermore, the larger nuclear spin and hyperfine strength of Si:Bi, compared with that of Si:P, are predicted to offer advantages for quantum information processing. Most notable amongst these is that magnetic field-dependent two-dimensional decoherence free subspaces, called optimal working points, have been identified to exist in Si:Bi, but not Si:P. 



==> acknowledgement.tex <==
I would like to give my thanks to the many people who have helped  me during the course of my Ph.D., and to whom I am greatly indebted.   My parents for their constant support during these years. My  colleagues and friends  with whom I had many stimulating conversations, not always about physics, which made my experience of Ph.D. life all the more richer.     Doctors Dara P. S.  McCutcheon and Ahsan Nazir for their guidance regarding open quantum systems. Doctors  Petra Leuders and In\'es G. Rubio for helping me with the experimental arts of magnetic resonance spectroscopy. And finally my supervisors, Professor Tania S. Monteiro and Doctor Gavin W. Morley, under whose mentorship I have grown as a physicist.        




==> declaration.tex <==
I, Mohammad Hamed Mohammady, declare that all work presented in this thesis, unless otherwise stated, is my own.  This work is based upon my published work in:

\begin{enumerate}[(i)]
\item
M. H. Mohammady, G. W. Morley, and T. S. Monteiro, ``\emph{Bismuth qubits in silicon: The role of EPR cancellation resonances}'', Phys. Rev. Lett., 105(6):067602, Aug 2010, doi:10.1103/PhysRevLett.105.067602.

\item M. H. Mohammady, G. W. Morley, A. Nazir, and T. S. Monteiro, ``\emph{Analysis of quantum coherence in bismuth-doped silicon: A system of strongly coupled spin qubits}'', Phys. Rev. B, 85:094404,
Mar 2012. doi: 10.1103/PhysRevB.85.094404.

\item S. J. Balian, M. B. A. Kunze, M. H. Mohammady, G. W. Morley, W. M. Witzel, C. W. M.
Kay, and T. S. Monteiro, ``\emph{Measuring central-spin interaction with a spin bath by pulsed ENDOR: Towards suppression of spin diffusion decoherence}'', Phys. Rev. B, 86:104428, Sep 2012.
doi: 10.1103/PhysRevB.86.104428.

\item G. W. Morley, P. Lueders, M. H. Mohammady, S. J. Balian, G. Aeppli, C. W. M. Kay, W. M.
Witzel, G. Jeschke, and T. S. Monteiro, ``\emph{Quantum control of hybrid nuclear-electronic qubits}'',
Nature Materials 12, 103-107, Jan 2013. doi: 10.1038/nmat3499.
\end{enumerate}

  





